Continual Source-Free Unsupervised Domain Adaptation

Existing Source-free Unsupervised Domain Adaptation (SUDA) approaches inherently exhibit catastrophic forgetting. Typically, models trained on a labeled source domain and adapted to unlabeled target data improve performance on the target while dropping performance on the source, which is not available during adaptation. In this study, our goal is to cope with the challenging problem of SUDA in a continual learning setting, i.e., adapting to the target(s) with varying distributional shifts while maintaining performance on the source. The proposed framework consists of two main stages: i) a SUDA model yielding cleaner target labels -- favoring good performance on target, and ii) a novel method for synthesizing class-conditioned source-style images by leveraging only the source model and pseudo-labeled target data as a prior. An extensive pool of experiments on major benchmarks, e.g., PACS, Visda-C, and DomainNet demonstrates that the proposed Continual SUDA (C-SUDA) framework enables preserving satisfactory performance on the source domain without exploiting the source data at all.

==> figures/figure_AblationStudy.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!h]
%
%\setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-5pt}
% \captionsetup{font=small}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.32\linewidth}
% \captionsetup{font=footnotesize}
\includegraphics[width=\linewidth]{figures/ssda_digit5_alpha_noise.png} 
\caption{}
\label{ablate:sub-1}
\end{subfigure}
%
\begin{subfigure}{.32\linewidth}
% \captionsetup{font=footnotesize}
\includegraphics[width=\linewidth]{figures/ssda_digit5_N_noise.png}
\caption{}
\label{ablate:sub-3}
\end{subfigure}
%
% \begin{subfigure}{.49\linewidth}
% \captionsetup{font=footnotesize}
% \includegraphics[width=\linewidth]{Images/ssda_digit5_N_noise.png}
% \caption{}
% \label{ablate:sub-3}
% \end{subfigure}
%
\begin{subfigure}{.32\linewidth}
% \captionsetup{font=footnotesize}
\includegraphics[width=\linewidth]{figures/ssda_digit5_N_AUG_RL_noise.png}
\caption{}
\label{ablate:sub-4}
\end{subfigure}
% \vspace{-0.5em}
\caption{Ablation study considering SVHN$\rightarrow$MNIST UDA task to determine optimal parameters of our proposed method.
(a): Single model is trained with $1$ label to choose the best $\alpha$ required to compute adaptive noise filtering threshold $\gamma$.
(b): Searching for the optimal number of members in the ensemble network. 
(c): Investigating the effect of labels and data augmentation type in all four possible scenarios. First and second letter of the legend represents label and augmentation type, respectively. Where S: Same and D: Different.
}
\vspace{-0.9em}
\label{fig:ablate_mclANDn}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> figures/figure_supp_domainnet.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[ht]
%
%\setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-5pt}
\captionsetup{font=small}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{0.3\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\textwidth]{figures/msda_domainnet_all_gamma.png}
\caption{Adaptiveness of $\gamma$ threshold.}
\label{DN:gamma}
\end{subfigure}
%
\begin{subfigure}{0.69\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\textwidth]{figures/Domainnet_noise.png}
\caption{Progressive noise reduction by pseudo-label refinement.}
\label{DN:noise}
\end{subfigure}
%
% \vspace{-0.5em}
\caption{Training evolution on DomainNet. Multi-source case: for each target, the rest of the domains are considered as source. For better representation, we concatenate noise reduction trends with different scales in (b). 
Legend: \textit{\textcolor{blue}{\textbf{C}}: Clipart, \textcolor{blue}{\textbf{I}}: Infograph, \textcolor{blue}{\textbf{P}}: Painting, \textcolor{blue}{\textbf{Q}}: Quickdraw, \textcolor{blue}{\textbf{R}}: Real, \textcolor{blue}{\textbf{S}}: Sketch, and \textcolor{blue}{\textbf{$\sigma$}}: Instantaneous standard deviation of three runs.}
}
% \vspace{-0.5em}
% \vspace{5em}
\label{DN:all}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> figures/figure_supp_neg.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
%
%\setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-5pt}
% \captionsetup{font=small}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hspace{0.2em}
\begin{subfigure}{0.3\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=0.8\linewidth]{figures/symm_hist.png}
\end{subfigure}
\hspace{0.6em}
\begin{subfigure}{0.3\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=0.8\linewidth]{figures/asymm_hist.png}
\end{subfigure}
\hspace{0.6em}
\begin{subfigure}{0.3\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=0.8\linewidth]{figures/shift_hist.png}
\end{subfigure}
% \\
% %
% \begin{subfigure}{0.32\textwidth}
% \centering
% \captionsetup{font=small}
% \includegraphics[width=\linewidth]{figures/symm_histogram_sep_epoch00350.jpg}
% \end{subfigure}
% \begin{subfigure}{0.32\textwidth}
% \centering
% \captionsetup{font=small}
% \includegraphics[width=\linewidth]{figures/asymm_histogram_sep_epoch00350.jpg}
% \end{subfigure}
% \begin{subfigure}{0.32\textwidth}
% \centering
% \captionsetup{font=small}
% \includegraphics[width=\linewidth]{figures/shift_histogram_sep_epoch00350.jpg}
% \end{subfigure}
\\
%
\begin{subfigure}{0.31\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\linewidth]{figures/symm_histogram_noisy_epoch00350.jpg}
% \caption{Symmetric-Noise}
% \label{NL:symm}
\end{subfigure}
\hspace{0.3em}
\begin{subfigure}{0.305\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\linewidth]{figures/asymm_histogram_noisy_epoch00350.jpg}
% \caption{Asymmetric-Noise}
% \label{NL:asymm}
\end{subfigure}
\hspace{0.3em}
\begin{subfigure}{0.305\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\linewidth]{figures/shift_histogram_noisy_epoch00350.jpg}
% \caption{Shift-Noise}
% \label{NL:shift}
\end{subfigure}
\\
%
\begin{subfigure}{0.315\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\linewidth]{figures/symm_histogram_clean_epoch00350.jpg}
\caption{Symmetric-Noise}
\label{NL:symm}
\end{subfigure}
% \hspace{2.25em}
\begin{subfigure}{0.317\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\linewidth]{figures/asymm_histogram_clean_epoch00350.jpg}
\caption{Asymmetric-Noise}
\label{NL:asymm}
\end{subfigure}
% \hspace{2.2em}
\begin{subfigure}{0.317\textwidth}
\centering
\captionsetup{font=small}
\includegraphics[width=\linewidth]{figures/shift_histogram_clean_epoch00350.jpg}
\caption{Shift-Noise}
\label{NL:shift}
\end{subfigure}
%
% \vspace{-0.5em}
\caption{Noise filtering capability of the existing Negative Learning method \cite{kim2019nlnl} over various noise distributions. Column (a) Symmetric Noise, column (b) Asymmetric artificial noise \cite{patrini2017making}, column (c) Shift noise \cite{morerio2020generative}. First row:  the confusion matrix shows how the noise is distributed in the beginning. Second row: confidence prediction for the noisy samples after training with NL. Third row: confidence prediction for the clean samples after training with NL. The amount of initial noise is same in magnitude (\textit{i.e.,} 32.97\%) for all the cases. Note that y-scales are different in the three cases}
% \vspace{-0.5em}
\label{NL:all}
\end{figure*}

==> tables/table_VisdaC_Full.tex <==
\begin{table*}[!t]
\centering
% \captionsetup{width=\linewidth,font=footnotesize}
\scriptsize
% \resizebox{\textwidth}{!}{
% \setlength{\abovecaptionskip}{-5pt}
% \setlength{\belowcaptionskip}{-5pt}
\begin{tabular}{|l|c c c c c c c c c c c c |c|}
\hline
Methods & \textcolor{blue}{\textbf{\textit{plane}}} & \textcolor{blue}{\textbf{\textit{bcycl}}} & \textcolor{blue}{\textbf{\textit{bus}}} & \textcolor{blue}{\textbf{\textit{car}}} & \textcolor{blue}{\textbf{\textit{horse}}} & \textcolor{blue}{\textbf{\textit{knife}}} & \textcolor{blue}{\textbf{\textit{mcycl}}} & \textcolor{blue}{\textbf{\textit{person}}} & \textcolor{blue}{\textbf{\textit{plant}}} & \textcolor{blue}{\textbf{\textit{skate}}} & \textcolor{blue}{\textbf{\textit{train}}} & \textcolor{blue}{\textbf{\textit{truck}}} & Avg.  \\
\hline
%
Inferred & 64.2 & 6.3 & 75.2 & 21.7 & 55.9 & 95.7 & 22.8 & 1.4 & 79.8 & 0.7 & 82.8 & 19.8 & 46.3  \\
\hline
% MCD \cite{saito2018maximum} & 87.0 & 60.9 & 83.7 & 64.0 & 88.9 & 79.6 & 84.7 & 76.9 & 88.6 & 40.3 & 83.0 & 25.8 & 71.9 \\
GPDA \cite{kim2019unsupervised} & 83.0 & 74.3 & 80.4 & 66.0 & 87.6 & 75.3 & 83.8 & 73.1 & 90.1 & 57.3 & 80.2 & 37.9 & 73.3 \\
% SAFN \cite{xu2019larger} & 93.6 & 61.3 & 84.1 & 70.6 & 94.1 & 79.0 & \textbf{91.8} & 79.6 & 89.9 & 55.6 & 89.0 & 24.4 & 76.1 \\
DADA \cite{tang2020discriminative} & 92.9 & 74.2 & 82.5 & 65.0 & 90.9 & \textbf{93.8} & 87.2 & 74.2 & 89.9 & 71.5 & 86.5 & 48.7 & 79.8 \\
% DSBN \cite{chang2019domain} & 94.7 & \textbf{86.7} & 76.0 & 72.0 & \textbf{95.2} & 75.1 & 87.9 & 81.3 & \textbf{91.1} & 68.9 & 88.3 & 45.5 & 80.2 \\
SHOT \cite{pmlr-v119-liang20a} & 94.3 & \textbf{88.5} & 80.1 & 57.3 & 93.1 & 94.9 & 80.7 & 80.3 & 91.5 & 89.1 & 86.3 & 58.2 & 82.9 \\
A$^2$Net \cite{Xia_2021_ICCV} & 94.0 & 87.8 & 85.6 & 66.8 & 93.7 & 95.1 & 85.8 & 81.2 & 91.6 & 88.2 & 86.5 & 56.0 & 84.3 \\
\hline
%
c$\rightarrow$Tg & 64.2 & 6.3 & 75.2 & 21.7 & 55.9 & 95.7 & 22.8 & 1.4 & 79.8 & 0.7 & 82.8 & 19.8 & 46.3  \\
%
% \hline
PLR (Tg) & \textbf{95.2} & 64.8 & \textbf{90.8} & \textbf{89.7} & 87.4 & 93.7 & \textbf{91.5} & \textbf{88.5} & 56.4 & 82.9 & \textbf{97.1} & \textbf{93.8} & \textbf{85.1} \\
%
\hline
SF-UDA (Tg) & \textbf{94.8} & 68.1 & \textbf{89.5} & \textbf{88.1} & 86.5 & 90.4 & \textbf{87.4} & \textbf{89.0} & 53.2 & 81.5 & \textbf{96.9} & \textbf{93.0} & \textbf{84.8}  \\
\textit{SF-UDA (Sc)} & \textit{45.2} & \textit{18.5} & \textit{55.9} & \textit{52.7} & \textit{54.8} & \textit{44.3} & \textit{12.5} & \textit{41.4} & \textit{24.6} & \textit{35.1} & \textit{40.2} & \textit{51.2} & \textit{39.7} \\
\hline
CSF-UDA (Tg) & \textbf{94.9} & 67.3 & \textbf{89.2} & \textbf{87.8} & 86.1 & 90.0 & 86.6 & \textbf{88.7} & 53.1 & 80.9 & \textbf{96.5} & \textbf{94.6} & \textbf{84.6} \\
\textit{CSF-UDA (Sc)} & \textit{\textbf{47.6}} & \textit{\textbf{21.4}} & \textit{\textbf{58.2}} & \textit{\textbf{54.3}} & \textit{\textbf{61.1}} & \textit{\textbf{49.5}} & \textit{\textbf{27.9}} & \textit{\textbf{41.9}} & \textit{\textbf{44.8}} & \textit{\textbf{36.2}} & \textit{\textbf{43.1}} & \textit{\textbf{55.4}} & \textit{\textbf{45.1}} \\
\hline
\end{tabular}
% }
% \vspace{-0.9em}
\caption{Classification accuracy on Visda-C with ResNet101.}
% \vspace{-0.9em}
\label{tab:VisdaC}
\end{table*}

==> tables/table_digit5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1.2} %<- modify value to suit your needs
\begin{table*}%[ht!]
\centering
% \captionsetup{width=\linewidth,font=scriptsize}
% \captionsetup{font=small}
\scriptsize
% \resizebox{0.9\textwidth}{!}{
% \setlength{\abovecaptionskip}{-20pt}
% \setlength{\belowcaptionskip}{-5pt}
\begin{tabular}{|l|c c c c c |c||l|c c c c c |c|}
\hline
\multicolumn{7}{|c||}{\textbf{Single-Source UDA}} & \multicolumn{7}{c|}{\textbf{Multi-Source UDA}} \\
\hline
\multirow{2}{*}{Sc} & 
\multirow{2}{*}{\textcolor{blue}{\textbf{\textit{T}}}} & 
\multirow{2}{*}{\textcolor{blue}{\textbf{\textit{T}}}} & 
\multirow{2}{*}{\textcolor{blue}{\textbf{\textit{T}}}} & 
\multirow{2}{*}{\textcolor{blue}{\textbf{\textit{S}}}} &
\multicolumn{1}{ c| }{\multirow{2}{*}{\textcolor{blue}{\textbf{\textit{U}}}}} & 
\multirow{3}{*}{Avg.} & 
&
\textcolor{blue}{\textbf{\textit{M,S,}}} & 
\textcolor{blue}{\textbf{\textit{T,S,}}} &
\textcolor{blue}{\textbf{\textit{T,M,}}} &
\textcolor{blue}{\textbf{\textit{T,M,}}} &
\multicolumn{1}{ c| }{\textcolor{blue}{\textbf{\textit{T,M,}}}} & 
\multirow{3}{*}{Avg.} 
\\
 & & & & & \multicolumn{1}{ c| }{ } & & 
&
\textcolor{blue}{\textbf{\textit{D,U}}} & 
\textcolor{blue}{\textbf{\textit{D,U}}} &
\textcolor{blue}{\textbf{\textit{D,U}}} &
\textcolor{blue}{\textbf{\textit{S,U}}} &
\multicolumn{1}{ c| }{\textcolor{blue}{\textbf{\textit{S,D}}}} & 
 
\\
\cline{1-6}
\cline{8-13}
Tg & 
\textcolor{blue}{\textbf{\textit{U}}} &
\textcolor{blue}{\textbf{\textit{S}}} &
\textcolor{blue}{\textbf{\textit{M}}} &
\textcolor{blue}{\textbf{\textit{T}}} &
\multicolumn{1}{ c| }{\textcolor{blue}{\textbf{\textit{T}}}} &
&
&
\textcolor{blue}{\textbf{\textit{T}}} &
\textcolor{blue}{\textbf{\textit{M}}} &
\textcolor{blue}{\textbf{\textit{S}}} &
\textcolor{blue}{\textbf{\textit{D}}} &
\multicolumn{1}{ c| }{\textcolor{blue}{\textbf{\textit{U}}}} & 
\\
\hline
% ATT \cite{pmlr-v70-saito17a} & -- & 52.8 & 94.0 & 85.8 & -- & -- & 
% DCTN \cite{xu2018deep} & -- & 70.9 & 77.5 & -- & -- & -- \\
SBA \cite{russo2018source} & 97.1 & 50.9 & \textbf{98.4} & 74.2 & 87.5 & 81.6 &
DCTN \cite{xu2018deep} & -- & 70.9 & 77.5 & -- & -- & --  \\
MALT \cite{minnehan2019deep} & 97.0 & \textbf{78.7} & 71.4 & 98.7 & 20.7 & 73.3 &
MM \cite{peng2019moment} & 98.4 & 72.8 & 81.3 & 89.5 & 96.1 & 87.6 \\
MTDA \cite{gholami2020unsupervised} & 94.2 & 52.0 & 85.5 & 84.6 & 91.5 & 81.5 &
OML \cite{li2020online} & 98.7 & 71.7 & 84.8 & 91.1 & 97.8 & 88.8 \\
GPLR \cite{morerio2020generative} & 89.3 & 63.4 & 94.3 & 97.3 & 91.8 & 87.5 &
CMSS \cite{yang2020curriculum} & 99.0 & 75.3 & 88.4 & 93.7 & 97.7 & 90.8 \\
SHOT \cite{pmlr-v119-liang20a} & \textbf{97.9} &  &  & 98.9 & 98.0 &  &
DECISION \cite{Ahmed_2021_CVPR} & \textbf{99.2} & 93.0 & 82.6 & \textbf{97.5} & 97.8 & 94.0 \\
 &  &  &  &  &  &  &
DRT \cite{li2021dynamic} & 81.0 & \textbf{99.3} & 86.6 & 93.8 & 98.4 & 91.8 \\
% \hline
% Source Only & 86.3 & 34.7 & 63.8 & 67.0 & 70.2 & 64.4 &
% & 98.7 & 69.1 & 52.1 & 40.4 & 88.8 & 69.8 \\
\hline
%
Sc$\rightarrow$Tg & 86.3 & 34.7 & 63.8 & 67.0 & 70.2 & 64.4 &
Sc$\rightarrow$Tg & 98.6 & 69.1 & 52.0 & 40.3 & 88.7 & 69.8 \\
% \hline
% AdaPLR$_{S1}$ & 86.3 &  &  &  &  &  &  &  &  &  &  &  &  \\
% AdaPLR$_{S2}$ & 99.1 &  &  &  &  &  &  &  &  &  &  &  &  \\
% PLR & \textbf{99.1} & 62.0 & 97.5 & \textbf{99.2} & \textbf{99.2} & \textbf{91.4} & 
% PLR & 98.8 & 94.2 & 84.6 & 87.8 & \textbf{98.6} & 92.8 \\
% \hline
SUDA & 97.4 & 61.6 & 95.4 & \textbf{99.2} & \textbf{99.2} & \textbf{90.6} & 
SUDA & 99.1 & 95.5 & \textbf{89.6} & 90.0 & 97.8 & \textbf{94.4} \\
% \textit{SF-UDA (Sc)} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} & 
% \textit{SF-UDA (Sc)} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} \\
% \hline
% CSF-UDA (Tg) &  &  &  &  &  &  & 
% CSF-UDA (Tg) &  &  &  &  &  &  \\
% \textit{CSF-UDA (Sc)} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} & 
% \textit{CSF-UDA (Sc)} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} & \textit{} \\
\hline
% Noise \textit{(init.)} & 39.0 & 75.1 & 73.5 & 3.9 & 41.8 & 56.0 & 48.2 & 21.5 & 22.1 & 4.0 & 35.4 & 20.8 \\
% Noise \textit{(rem.)} & 18.9 & 23.1 & 68.3 & 1.81 & 19.0 & 48.8 & 30.0 & 10.7 & 12.8 & 1.9 & 16.8 & 10.6 \\
% \hline
\end{tabular}
% }
% \vspace{-0.5em}
\caption{Classification accuracy on Digit5 with a naive 3-layer CNN. C-SUDA is not reported due to the limitation of the naive 3-layer CNN (More details in Sec. E of Supplementary Material.).
%Source Only: inferred pseudo-labels accuracy,
Legend: \textit{
% \textbf{Sc:} Source (real), \textbf{Tg:} Target (real), \textbf{Sc$\rightarrow$Tg}: Inferred pseudo-labels, \textbf{PLR}: Pseudo-label refinement (output of Stage 1), \textbf{SUDA:} Source-free UDA, 
\textcolor{blue}{\textbf{T}}: MNIST, \textcolor{blue}{\textbf{S}}: SVHN, \textcolor{blue}{\textbf{U}}: USPS, \textcolor{blue}{\textbf{M}}: MNIST-M, and \textcolor{blue}{\textbf{D}}: Synthetic-digits.}}
% \vspace{-3.0em}
\label{tab:digit5}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}%[ht]
% \setlength{\abovecaptionskip}{-5pt}
% % \setlength{\belowcaptionskip}{-5pt}
% \begin{center}
% \begin{tabular}{|l c c c c c c c|}
% \hline
% Methods & \textcolor{blue}{\textbf{\textit{P}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{A}}} & \textcolor{blue}{\textbf{\textit{P}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{C}}} & \textcolor{blue}{\textbf{\textit{P}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{S}}} & \textcolor{blue}{\textbf{\textit{A}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{P}}} &
% \textcolor{blue}{\textbf{\textit{A}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{C}}} &
% \textcolor{blue}{\textbf{\textit{A}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{S}}} & Avg \\
% \hline
% 1-NN \cite{gholami2020unsupervised} & 15.2 & 18.1 & 25.6 & 22.7 & 19.7 & 22.7 & 20.7 \\
% ADDA \cite{gholami2020unsupervised} & 24.3 & 20.1 & 22.4 & 32.5 & 17.6 & 18.9 & 22.6 \\
% DSN \cite{gholami2020unsupervised}  & 28.4 & 21.1 & 25.6 & 29.5 & 25.8 & 24.6 & 25.8 \\
% MTDA \cite{gholami2020unsupervised} & 31.4 & 23.0 & 28.2 & 35.7 & 27.0 & 28.9 & 29.0 \\
% \hline
% Ours & \textbf{82.6}$\pm$0.83 & \textbf{80.5}$\pm$2.66 & \textbf{32.3}$\pm$0.68 & \textbf{98.4}$\pm$0.03 & \textbf{84.3}$\pm$1.50 & \textbf{56.1}$\pm$1.27 & \textbf{72.4}$\pm$1.20 \\
% \hline
% Noise \textit{(initial)} & 39.0 & 75.1 & 73.5 & 3.9 & 41.8 & 56.0 & 48.2 \\
% Noise \textit{(remaining)} & 18.9$\pm$0.44 & 23.1$\pm$1.36 & 68.3$\pm$0.97 & 1.81$\pm$0.19 & 19.0$\pm$0.77 & 48.8$\pm$1.03 & 30.0$\pm$0.8 \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Add caption (e.g., SSDA: PACS)}
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}%[ht]
% \setlength{\abovecaptionskip}{-5pt}
% % \setlength{\belowcaptionskip}{-5pt}
% \begin{center}
% \begin{tabular}{|l c c c c c|}
% \hline
% Methods & \textcolor{blue}{\textbf{\textit{C, P, S}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{A}}} & \textcolor{blue}{\textbf{\textit{A, P, S}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{C}}} & \textcolor{blue}{\textbf{\textit{A, C, S}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{P}}} & \textcolor{blue}{\textbf{\textit{A, C, P}}} $\rightarrow$ \textcolor{blue}{\textbf{\textit{S}}} & Avg \\
% \hline
% DDiscovery \cite{mancini2018boosting} & 87.5 & 87.0 & 96.6 & 71.6 & 85.7 \\
% SIB \cite{Hu2020Empirical} & 88.9 & 89.0 & 98.3 & 82.2 & 89.6 \\
% Meta-MCD \cite{li2020online} & 87.4 & 86.1 & 97.1 & 78.2 & 87.2 \\
% RABN \cite{xu2019self} & 86.8 & 86.5 & 98.01 & 71.5 & 85.7 \\
% JiGen \cite{carlucci2019domain} & 84.8 & 81.0 & 97.9 & 79.0 & 85.7 \\
% % \cite{ganin2015unsupervised} & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
% %MDAN \cite{zhao2018adversarial}   & 79.1$\pm$0.36 & 76.0$\pm$0.73 & 91.4$\pm$0.85 & 72.0$\pm$0.80 & 79.6$\pm$0.69 \\
% %DANN \cite{ganin2015unsupervised} & 81.9$\pm$1.13 & 77.5$\pm$1.26 & 91.8$\pm$1.21 & 74.6$\pm$1.03 & 81.5$\pm$1.16 \\
% %MCD \cite{saito2018maximum}       & 88.7$\pm$1.01 & 88.9$\pm$1.53 & 96.4$\pm$0.42 & 73.9$\pm$3.94 & 87.0$\pm$1.73 \\
% %M$^3$SDA \cite{peng2019moment}    & 89.3$\pm$0.42 & 89.9$\pm$1.00 & 97.3$\pm$0.31 & 76.7$\pm$2.86 & 88.3$\pm$1.15 \\
% CMSS \cite{yang2020curriculum} & 88.6$\pm$0.36 & \textbf{90.4}$\pm$0.80 & 96.9$\pm$0.27 & 82.0$\pm$0.59 & 89.5$\pm$0.50 \\
% \hline
% Ours & \textbf{90.8}$\pm$0.08 & 89.5$\pm$0.54 & \textbf{98.8}$\pm$0.12 & \textbf{85.2}$\pm$0.73 & \textbf{91.1}$\pm$0.73 \\
% \hline
% Noise \textit{(initial)} & 21.5 & 22.1 & 4.0 & 35.4 & 20.8 \\
% Noise \textit{(remaining)} & 10.7$\pm$0.36 & 12.8$\pm$0.15 & 1.9$\pm$0.23 & 16.8$\pm$0.86 & 10.6$\pm$0.40 \\
% \hline
% \end{tabular}
% \end{center}
% \caption{Add caption (e.g., MSDA: PACS)}
% \end{table*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}%[ht]
% \setlength{\abovecaptionskip}{-5pt}
% % \setlength{\belowcaptionskip}{-5pt}
% \begin{center}
% \begin{tabular}{|l |c c c c c c|c|c c c c|c|}
% \hline
% & \multicolumn{7}{ c| }{\textbf{Multi-Target UDA}} & \multicolumn{5}{ c| }{\textbf{Multi-Source UDA}} \\
% \hline
% Source & 
% \textcolor{blue}{\textbf{\textit{P}}} & 
% \textcolor{blue}{\textbf{\textit{P}}} & 
% \textcolor{blue}{\textbf{\textit{P}}} & 
% \textcolor{blue}{\textbf{\textit{A}}} &
% \textcolor{blue}{\textbf{\textit{A}}} &
% \textcolor{blue}{\textbf{\textit{A}}} & 
% \multirow{2}{*}{Avg.} & 
% \textcolor{blue}{\textbf{\textit{C,P,S}}} & 
% \textcolor{blue}{\textbf{\textit{A,P,S}}} &
% \textcolor{blue}{\textbf{\textit{A,C,S}}} &
% \textcolor{blue}{\textbf{\textit{A,C,P}}} & 
% \multirow{2}{*}{Avg.} 
% \\
% \cline{1-7}
% \cline{9-12}
% Target & 
% \textcolor{blue}{\textbf{\textit{A}}} &
% \textcolor{blue}{\textbf{\textit{C}}} &
% \textcolor{blue}{\textbf{\textit{S}}} &
% \textcolor{blue}{\textbf{\textit{P}}} &
% \textcolor{blue}{\textbf{\textit{C}}} &
% \textcolor{blue}{\textbf{\textit{S}}} &
% &
% \textcolor{blue}{\textbf{\textit{A}}} &
% \textcolor{blue}{\textbf{\textit{C}}} &
% \textcolor{blue}{\textbf{\textit{P}}} &
% \textcolor{blue}{\textbf{\textit{S}}} & 
% \\
% \hline
% 1-NN \cite{gholami2020unsupervised} & 15.2 & 18.1 & 25.6 & 22.7 & 19.7 & 22.7 & 20.7 &  --  &  --  &  --  &  --  &  -- \\
% ADDA \cite{gholami2020unsupervised} & 24.3 & 20.1 & 22.4 & 32.5 & 17.6 & 18.9 & 22.6 &  --  &  --  &  --  &  --  &  -- \\
% DSN \cite{gholami2020unsupervised}  & 28.4 & 21.1 & 25.6 & 29.5 & 25.8 & 24.6 & 25.8 &  --  &  --  &  --  &  --  &  -- \\
% MTDA \cite{gholami2020unsupervised} & 31.4 & 23.0 & 28.2 & 35.7 & 27.0 & 28.9 & 29.0 &  --  &  --  &  --  &  --  &  -- \\
% DD \cite{mancini2018boosting}       &  --  &  --  &  --  &  --  &  --  &  --  &  --  & 87.5 & 87.0 & 96.6 & 71.6 & 85.7 \\
% SIB \cite{Hu2020Empirical}          &  --  &  --  &  --  &  --  &  --  &  --  &  --  & 88.9 & 89.0 & 98.3 & 82.2 & 89.6 \\
% MMCD \cite{li2020online}            &  --  &  --  &  --  &  --  &  --  &  --  &  --  & 87.4 & 86.1 & 97.1 & 78.2 & 87.2 \\
% RABN \cite{xu2019self}              &  --  &  --  &  --  &  --  &  --  &  --  &  --  & 86.8 & 86.5 & 98.0 & 71.5 & 85.7 \\
% JiGen \cite{carlucci2019domain}     &  --  &  --  &  --  &  --  &  --  &  --  &  --  & 84.8 & 81.0 & 97.9 & 79.0 & 85.7 \\
% CMSS \cite{yang2020curriculum}      &  --  &  --  &  --  &  --  &  --  &  --  &  --  & 88.6 & \textbf{90.4} & 96.9 & 82.0 & 89.5 \\
% \hline
% Inferred & 61.0 & 24.9 & 26.6 & 96.1 & 58.2 & 44.0 & 51.8 & 78.5 & 77.9 & 96.0 & 64.6 & 79.2 \\
% \hline
% AdaPLR & \textbf{82.6} & \textbf{80.5} & \textbf{32.3} & \textbf{98.4} & \textbf{84.3} & \textbf{56.1} & \textbf{72.4} & \textbf{90.8} & 89.5 & \textbf{98.8} & \textbf{85.2} & \textbf{91.1} \\
% \hline
% % Noise \textit{(init.)} & 39.0 & 75.1 & 73.5 & 3.9 & 41.8 & 56.0 & 48.2 & 21.5 & 22.1 & 4.0 & 35.4 & 20.8 \\
% % Noise \textit{(rem.)} & 18.9 & 23.1 & 68.3 & 1.81 & 19.0 & 48.8 & 30.0 & 10.7 & 12.8 & 1.9 & 16.8 & 10.6 \\
% % \hline
% \end{tabular}
% \end{center}
% \caption{Add caption (e.g., PACS)}
% \end{table*}
